Human Grasp Classification for Reactive Human-to-Robot Handovers

Transfer of objects between humans and robots is a critical capability for collaborative robots. Although there has been a recent surge of interest in human-robot handovers, most prior research focus on robot-to-human handovers. Further, work on the equally critical human-to-robot handovers often assumes humans can place the object in the robot's gripper. In this paper, we propose an approach for human-to-robot handovers in which the robot meets the human halfway, by classifying the human's grasp of the object and quickly planning a trajectory accordingly to take the object from the human's hand according to their intent. To do this, we collect a human grasp dataset which covers typical ways of holding objects with various hand shapes and poses, and learn a deep model on this dataset to classify the hand grasps into one of these categories. We present a planning and execution approach that takes the object from the human hand according to the detected grasp and hand position, and replans as necessary when the handover is interrupted. Through a systematic evaluation, we demonstrate that our system results in more fluent handovers versus two baselines. We also present findings from a user study (N = 9) demonstrating the effectiveness and usability of our approach with naive users in different scenarios. More results and videos can be found at http://wyang.me/handovers.

==> 06experiments-backup.tex <==
In this section, we first evaluate the performance of human grasp classification that was discussed in Sec. ~\ref{section:hand_model}.
% and compare it with using object detection to determine whether there is an object in the human hand. 
Then we perform two sets of handover experiments: one systematic evaluation, where we compare to several baseline approaches, and a user study to determine how effectively our system allowed users to make human-robot handovers under different conditions.
% We assess our system in several ways. First, we assess our model from Sec.~\ref{section:hand_model} on a held-out test dataset, compared to using object detection to determine if we should grasp an object. Second, we perform two sets of handover experiments: one systematic evaluation, where we compare to several baseline approaches, and a user study to determine how effectively our system allowed users to make human-robot handovers under different conditions.

\subsection{Evaluation of Human Grasp Classification}
% here we describe performance of the hand grasp classification model on its own.

% \begin{table}[bt]
%     \centering
%     \caption{Accurary (\%) of hand state classification.}
%     \label{tab:hand-classification}
%     %\begin{tabular}{l c c c c c c c c}
%     %    \toprule
%     %     & Holding & Pinch-bottom & Pinch-top & Pinch-side & lifting & Waiting & Idle & Mean \\
%     %     \midrule
%     %     Accuracy & 90.1 & 90.3 & 83.2 & 96.3 & 57.4 & 79.8 & 57.5 & 78.8 \\
%     %     \bottomrule
%     \begin{tabular}{l c}
%     \toprule
%     on-open-palm & 90.1 \\
%     Pinch-bottom & 90.3 \\
%     Pinch-top & 83.2 \\
%     Pinch-side & 96.3 \\
%     Lifting & 57.4 \\
%     Waiting & 79.8 \\
%     Others & 57.5 \\
%     \midrule
%     Mean & 78.9 \\
%     \bottomrule
%     \end{tabular}
% \end{table}


We evaluate our hand grasp classification model on a validation set collected with a subject which is unseen during the training procedure. The classification accuracy is reported in Fig~\ref{fig:acc_detection_rate} (a), which demonstrates the good generalization ability of our model on unseen subjects.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/detection_rate.pdf}
    \caption{
    (a) The accuracy of the human hand grasp classification. 
    (b) The comparison of the object miss-detection rate between our hand states classification and PoseCNN~\cite{xiang2017posecnn}. In many cases the hand occludes the object, meaning that it is very difficult to get an accurate pose estimate. 
    % \cpax{Mean is not very meaningful, maybe remove. --resolved}
    }
    \vspace{-1em}
    \label{fig:acc_detection_rate}
\end{figure}

We also conduct an experiment to evaluate the detection rate, \ie, whether there is an object in the hand, to give us an insight on how robust the handover system is against the occlusion. 
We compare the detection rate of our hand grasp classification model (with/without object) to that of a state-of-the-art object detection method~\cite{xiang2017posecnn}. 
The result is reported in Fig.~\ref{fig:acc_detection_rate}(b). 
We can see that our human grasp model is more robust compared with~\cite{xiang2017posecnn}, especially when heavy occlusion occurs (\eg, $87.5\%$ \vs $6.8\%$ for  \textit{pinch-side} and $94.4\%$ \vs $11.9\%$ for \textit{lifting}).
% For PoseCNN~\cite{}, the missing detection is happened when the object is in the scene while the detection is missing. 
% For hand state classification based inference, the missing detection if defined when the hand is grasping an object while the classifier predicts ``waiting" or ``idle" states. 
% From Fig.~\ref{} we can see that 
% our classification model has lower miss-detection rate due to its robustness against occlusion??? (TODO: need to verify)


%\subsection{Handover Experiment}
\subsection{Systematic and Usability Experiments}

%\begin{figure}
%    \centering
%    % \includegraphics{}
%    \caption{Experimental setup for the human-robot block handoff task. The robot must be able to either take robots from a %human or give blocks to a human, depending on the needs of the task.}
%    \label{fig:franka}
%\end{figure}

In this subsection, we describe the systematic evaluation and the usability study we conducted on our handover system. 
The experiments are set up so that a robot is mounted on the table, as shown in Fig.~\ref{fig:task-plan}. A human user is going to hand four colored blocks over to the robot, one at a time. 

% First, we compared our system to several baselines, in order to see if our system is better and more responsive than certain baselines.
%  We did two experiments: a systematic evaluation and a usability study.

%During the systematic evaluation, we tested each of three systems
\subsubsection{Systematic Evaluation.}
First, we compared our system to several baselines, in order to see if our system is better and more responsive than certain baselines.
During the systematic evaluation, we tested each of three approaches for determining which grasp pose to use for taking an object from the human:

\textbf{Simple Baseline}: %A baseline version of the system, which 
waits until it sees the block in a human hand and takes it from the hand, using a fixed grasp orientation. The human hand is detected via an off-the-shelf system; in our case, the Microsoft Azure body tracker~\cite{k4a}.
    
\textbf{Hand Pose Estimation}: A state estimation-based version of the system, in which we use the human hand pose from the Azure body tracker to infer grasp direction. %and use this to infer the grasp direction.
    
\textbf{Ours}: The proposed system, classifying human grasps based on depth information as described in Sec.~\ref{section:hand_model}.
%\end{itemize}

All variants executed the same task model, as described in Sec.~\ref{section:task_model}. The order in which these three test cases were provided was randomized. %All users were given two minutes to acclimate to the system, and then told to hand each of the four blocks over to the robot, one at a time.
Users used their right hand to present blocks to the robot. We then computed the metrics from Sec.~\ref{ssec:metrics}.

%We gave all users two minutes (120 seconds) to ``warm up'' with each system. We instructed users to hold their hand still when they want the robot to take the block. If the robot cannot grasp the block, try moving it, but remember that the robot will not grasp the object if it is moving. Each block was assigned a particular grasp: (1) holding, (2) pinch bottom, (3) pinch top, (4), pinch side, and (5) lifting. Users were instructed to use their warm up time to try each grasp. We give them a maximum time of 60 seconds per grasp; after this period, we moved on.

\subsubsection{Usability Study.} 
We also performed an usability study, for which we recruited nine users, ages $20$ to $36$. Of these, two were female and seven were male. The average age was $30.44 \pm 4.74$ years. 
The study consisted of three rounds:

\textbf{Freeform}: first, users were given four blocks and instructed to stand in front of the table and hand the blocks over to the robot one at a time. They were instructed that the robot would only take blocks if their hand is still, but they could hold the blocks any way they liked.

\textbf{Attentive}: %After the first round of the user study, we then
Next we demonstrated the set of five human grasps %defined in our dataset
shown in Fig.~\ref{fig:grasp_types}: \textit{pinch-top, pinch-bottom, pinch-side, lifting}, and \textit{on-open-palm}. We then told the participants to hand over four blocks again. %This time, 
We encouraged them to try the predefined hand grasps, but they were able to use any others.
    
\textbf{Distracted}: Finally, we tested user performance in the presence of a distraction. Users watched a music video on YouTube \footnote{\url{https://youtu.be/4jd6dNrJRh4}} and counted the number of faces that appeared, while handing over all four blocks to the robot.
%\end{itemize}

%You can hold the blocks any way you like, whatever feels comfortable. It will move slowly and is human-safe. It may take a moment for the robot to realize you are trying to hand a block over, but you may move your hand to a new position or change the way you are holding a block if it seems stuck. First, do you have any questions?"

%Our usability study aims to take naive users and determine how 


%We have a Franka Panda robot arm mounted on a table, as shown in Fig.~\ref{fig:task-plan}. The goal is for the robot to pick up blocks from the human and put them in a bin to its left. The robot will then take a block of a different color and hand it over to the human.

%The human is busy performing a simple task on the computer. When alerted, they have to take a block from the robot. When alerted a different way, they need to give a specific block to the robot. If they give the robot the wrong block, then the robot will reject it and give the block back maybe?

% \noindent\textbf{Test subjects.} We recruited nine users, ages $20$ to $36$. Of these, two were female and seven were male. The average age was $30.44 \pm 4.74$ years.

\subsection{Evaluation Metrics} \label{ssec:metrics}

% --------
\subsubsection{Systematic Evaluation}
We evaluate the system performance with a set of metrics computed during trials. 

%\begin{itemize}
%    \item \textbf{Planning Success Rate}: 
%    \item \textbf{Grasp Success Rate}: 
%    \item \textbf{Action Execution Time}
%    \item \textbf{Total Execution Time}:
%    \item \textbf{Trial Duration}: 
%\end{itemize}
\textbf{Planning Success Rate:}
%First, we compute the ``approach'' success rate. This is 
the number of times the \texttt{follow\_plan} operator was able to execute successfully, bringing the robot to its standoff pose, and measures certainty both of the human and the system. % attempts versus the total number of blocks -- this give us\wei{?}

\textbf{Grasp Success Rate:} how often the robot was able to successfully take the object from the human, versus total number of grasp attempts that it made.

\textbf{Action execution Time:} tracks the amount of time it took to execute a single planned trajectory, grasp a block, and place it on the table. This is higher if the robot must take a longer path to grasp the block from the human.

\textbf{Total Execution Time:} the amount of time it took to execute all planned paths, including replanning because the human moved or because grasp classification changed.

\textbf{Trial Duration:} Time since human hand was first detected until the trial was complete.

%Finally, we look at time to successful grasp for each block. This is counted from the moment that the human first enters the robot's workspace with a particular block.

\subsubsection{Usability Study} During the usability study, we counted the following statistics: a) number of times robot gripper contacted human fingers, b) number of times users changed their grasps, and c) number of times they changed hand position.
%
%\textbf{Questions.}
After all three trials were done, we gave users a Likert scale questionnaire.
%for their thoughts about the differences between the different systems and which ones they preferred. We gave them a Likert scale questionnaire. %We lso asked how it was different from handing from a human, and asked other specific followup questions


\subsection{Results}

\begin{table*}[bt]
    \centering
    \caption{Results for handover performance on our quantitative metrics. Planning success rate indicates how often the system needed to replan its approach, versus grasp success rate as the number of times the system successfully took the object.}
    \label{tab:hand-tracking}
    \begin{tabular}{l c c c c c}
        \toprule
         & Planning Success Rate & Grasp Success Rate & Action Execution Time (s) & Total Execution Time (s) & Trial Duration (s) \\
         \midrule
         % No Reactive Execution & &  & \\
         %Fixed Grasp Position &  &  & \\
         Simple Baseline & 42.1\% & 66.7\% & 11.37 & 20.93 & 21.59 \\
         Hand Pose Estimation & 29.6\% & 80.0\% & 15.10 & 36.34 & 36.46 \\
         Ours & 64.3\% & 100\% & 13.20 & 17.34 & 18.31 \\
         \bottomrule
    \end{tabular}
\end{table*}


\subsubsection{Systematic Evaluation}
Table~\ref{tab:hand-tracking} shows results on each of our main metrics during the systematic evaluation.
Our method consistently improves the success rate and reduces the total execution time and the trial duration compared with the two other baseline methods, which proves the efficacy and the reliability of our method. 

The only exception is the \textit{Action Execution Time}, where the \textit{simple baseline} is often faster. This is because the simple baseline does not plan as adaptively as the others; it would not try to attempt an unusual grasp. This means that time from a successful approach to dropping the object is, on average, notably lower.

%Users did notice the difference. They said that the grasp attempts from the grasp classification system seemed to be more considerate; they would ``need to move their hand out of the way less.''

\subsubsection{Usability Study}
Fig.~\ref{fig:likert_scale} shows the results of the questionnaire given to our study participants. There was a range of responses, but users said that they worked fluently with the robot and trusted it to do the right thing, although they noted several common issues when asked for feedback. They also believed that the robot was aware of their actions.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/likert_scale_v2.pdf}
    \caption{Results form the Likert scale questionaire given to users during the usability study. Users thought they worked together fluently with the robot, although there were several issues. Users were asked questions at the end of the study.}
    \label{fig:likert_scale}
\end{figure}

\begin{table*}[bt]
    \centering
    \caption{Quantitative results from the user study. Users were able to complete tasks quickly even when they were distracted and had to concentrate on a different scenario.}
    \label{tab:study}
    \begin{tabular}{l c c c c c}
        \toprule
         & Planning Success Rate & Grasp Success Rate & Action Execution Time (s) & Total Execution Time (s) & Trial Duration (s) \\
         \midrule
         % No Reactive Execution & &  & \\
         %Fixed Grasp Position &  &  & \\
         Freeform & 32.7\% & 67.3\% & 13.21 & 25.99 & 26.92 \\
         Attentive & 40.0\% & 90.0\% & 14.85 & 23.84 & 24.75 \\
         Distracted & 29.8\% & 67.9\% & 11.08 & 26.08 & 27.02 \\
         \midrule
         Overall & 33.6\% & 73.6\% & 13.05 & 25.31 & 26.24 \\
         \bottomrule
    \end{tabular}
\end{table*}

We also computed our quantitative metrics on user data, as seen in Table~\ref{tab:study}. Approaches and grasps were less successful when users were distracted, but times are similar.
Users counted an average of $12.88 \pm 3.48$ faces in the music video, when the correct number was $13$. This implies many of them felt certain level of confident of the handover system and were paying a good amount of attention to the video.


==> 07discussion.tex <==
\begin{figure}[bt]
    \centering
    \includegraphics[width=0.21\textwidth]{figures/user_study_grasp_type_1st.pdf}
    \includegraphics[width=0.21\textwidth]{figures/user_study_grasp_type_2nd.pdf}
    \includegraphics[width=0.21\textwidth]{figures/user_study_grasp_type_3rd.pdf}
    \includegraphics[width=0.21\textwidth]{figures/user_study_other_statistic.pdf}
    \caption{
    Coverage of human grasps during the usability study. \textit{Others} denotes the user grasps that are not included in our human grasp dataset. 
    Our human grasp dataset covers $77\%$ of the user grasps even  before the users were informed the ways of grasp included in our system (see \textit{Freeform}). We also report the average times that the users repositioned their hand, changed the way of grasp, and were contacted by the gripper. 
    }
    \label{fig:user_study_statistics}
\end{figure}

\begin{figure}[bt]
	\centering
	\small
	%\begin{tabular}{c c c c c}
	%	\includegraphics[width=0.16\textwidth]{figures/outliers/01.png} &
	%	\includegraphics[width=0.16\textwidth]{figures/outliers/02.png} &
	%	\includegraphics[width=0.16\textwidth]{figures/outliers/03.png} &
	%	\includegraphics[width=0.16\textwidth]{figures/outliers/04.png} &
	%	\includegraphics[width=0.16\textwidth]{figures/outliers/05.png} \\
	%	(a) & (b) & (c) & (d) & (e)
	%\end{tabular}
    \includegraphics[width=0.24\linewidth]{figures/outliers/01.png}
	\includegraphics[width=0.24\linewidth]{figures/outliers/02.png}
	\includegraphics[width=0.24\linewidth]{figures/outliers/03.png}
	\includegraphics[width=0.24\linewidth]{figures/outliers/04.png} 
% 	\includegraphics[width=0.14\textwidth]{figures/outliers/05.png}
	
% 	\vspace{-1em}
	\caption{Outliers grasps which do not appear in our training dataset, and are examples of the types of grasps where our system showed higher uncertainty, leading to slightly worse handover performance.}
	\label{fig:outliers}
\end{figure}

First, we report the coverage of different ways of grasp during the usability study in Fig.~\ref{fig:user_study_statistics}. 
In general, our definition of human grasps covers $77\%$ of the user grasps even before they know the ways of grasps defined in our system (see \textit{Freeform} in Fig.~\ref{fig:user_study_statistics}, which proves a good coverage of our human grasp design. 
While our system can deal most of the unseen human grasps, they tend to lead to higher uncertainty and sometimes would cause the robot to backoff and replan.
Some of these unseen grasps are shown in Fig.~\ref{fig:outliers}. This suggests directions for future research; ideally we would be able to handle a wider range of grasps that a human might want to use.

We also report the average number of times that users repositioned their hand, changed their way of grasp, and were contacted by the gripper in Fig.~\ref{fig:user_study_statistics}. 
During the final, distracted test, users had to reposition or change their ways of grasp more often compared with the first two rounds. 
Several complained about their fingers being pinched, or saw the robot fail to grasp objects. One specifically ``chose to use the palm-facing-up hand pose'' to minimize risk of failure; another ``had to look at the robot every 10s or so.'' 

This issue came up for several reasons. One of the most important is that many of the grasp poses are very hard for the robot to reach -- they are at the edges of its configuration space, and may require some complex motions to get there. 
% Second, the users could also reposition their hands unintentionally while being distracted. 
In the future, we should strive to make the whole system more legible, indicating which blocks the robot wants to move to and how it wants to get there~\cite{dragan2013legibility}. 

In general, our users quickly noticed that the robot was trying to grab the block in an unobtrusive way as possible. 
They also noted a slight inaccuracy during the robot's grasps and approaches, but this doesn't seem to have been a major issue. One said about the robot ``it may require my assistance in slightly moving towards where it expected the goal to be.'' In other words, even though the robot's grasp pose might be slightly off due to an inaccurate hand pose or occluded object, the robot and human together were reliably able to execute the handoff.

From a usability perspective, our trajectories weren't always totally legible. The underlying motion planner used in Sec.~\ref{section:task_model} was based on RRT-connect~\cite{kuffner2000rrt}, and sometimes it would make surprising choices to reach grasp positions. For example, one user said after the first experiment, ``There was one of the trajectories that had a small detour.'' Another said ``Holding the block in such a way that the robot needed to rotate its grasp 90 degrees seemed to cause problems.'' This is because the robot would often be unclear about what the position and orientation of the hand was, and would end up being uncertain. In the end, the motion plans could be hard to interpret -- ``I was still unsure of what the actual behavior will be like.''

Users did notice that after the second round of experiments, when they were shown how to grasp the objects, that the system was more reliable and easier to work with. One users said ``the estimate of the object/hand position seemed more precise'' after they were taught these grasps. % particular grasps to us.

During the final, distracted test, users were more nervous. Several complained about their fingers being pinched, or saw the robot fail to grasp objects. One specifically ``chose to use the palm-facing-up hand pose'' to minimize risk of failure; another ``had to look at the robot every 10s or so.'' 

This issue came up for several reasons. First, many of the grasp poses are very hard for the robot to reach -- they are at the edges of its configuration space, and may require some complex motions to get there. 
Second, the users could also reposition their hands unintentionally while being distracted. 
In the future, we should strive to make the whole system more legible, indicating which blocks the robot wants to move to and how it wants to get there~\cite{dragan2013legibility}. 
% In addition, sometimes the object is not visible -- if we cannot detect any object pixels, the robot will be much less accurate\wei{TBD}.
